Tight FPT Approximation for Socially Fair Clustering

In this work, we study the socially fair $k$-median/$k$-means problem. We are given a set of points $P$ in a metric space $\mathcal{X}$ with a distance function $d(.,.)$. There are $\ell$ groups: $P_1,\dotsc,P_{\ell} \subseteq P$. We are also given a set $F$ of feasible centers in $\mathcal{X}$. The goal in the socially fair $k$-median problem is to find a set $C \subseteq F$ of $k$ centers that minimizes the maximum average cost over all the groups. That is, find $C$ that minimizes the objective function $\Phi(C,P) \equiv \max_{j} \Big\{ \sum_{x \in P_j} d(C,x)/|P_j| \Big\}$, where $d(C,x)$ is the distance of $x$ to the closest center in $C$. The socially fair $k$-means problem is defined similarly by using squared distances, i.e., $d^{2}(.,.)$ instead of $d(.,.)$. The current best approximation guarantee for both the problems is $O\left( \frac{\log \ell}{\log \log \ell} \right)$ due to Makarychev and Vakilian [COLT 2021]. In this work, we study the fixed parameter tractability of the problems with respect to parameter $k$. We design $(3+\varepsilon)$ and $(9 + \varepsilon)$ approximation algorithms for the socially fair $k$-median and $k$-means problems, respectively, in FPT (fixed parameter tractable) time $f(k,\varepsilon) \cdot n^{O(1)}$, where $f(k,\varepsilon) = (k/\varepsilon)^{{O}(k)}$ and $n = |P \cup F|$. Furthermore, we show that if Gap-ETH holds, then better approximation guarantees are not possible in FPT time.

==> improved_fpt_bound.tex <==
\section{Improved FPT Running Time}

In this subsection, we show that the socially fair clustering problem admits an $e^{O(p)}/\gamma$ approximation algorithm with the running time $(1/(1-\gamma))^{k} \cdot n^{O(1)}$. We convert the bi-criteria $(e^{O(p)}/\gamma,1/(1-\gamma))$-approximation algorithm of Makarychev and Vakilian~\cite{fairness:2021_Socially_Makarychev)} to an FPT algorithm.

\begin{lemma}
Let $C$ be an $(\alpha,\beta)$-approximate solution to the socially fair clustering problem. Then, there exist a $k$ sized subset $C'$ of $C$ that gives $O(\alpha)$-approximation guarantee. 
\end{lemma}

\begin{proof}
Let $C^{*} = \{c_{1}^{*},\dotsc,c_{k}^{*} \}$ be an optimal center set. This center set induces a Voronoi partitioning of the point set $P$. Let the partitions are $\mathcal{P}_1,\dotsc,\mathcal{P}_k$. This center set also induces a Voronoi partitioning in each of the groups. 
We denote this partitioning using the notation $\mathbb{P}_{j} = \{P_j^1,P_j^2, \dotsc,P_j^k\}$ for the $j^{\textrm{th}}$ group. 
That is, $P_j^i$ are the set of those points in group $P_j$ for which the center $\cpst{i}$ is the closest. Also note that $\mathcal{P}_i = P_{1}^{i} \cup \dotsc \cup P_{\ell}^{i}$. 

\noindent For every partition $\mathcal{P}_{i}$, we define a  \emph{representative} client $x^{*}_{i} \in C_{i}$ as follows:
\[
x_{i}^{*} \coloneqq \arg\min_{x \in \mathcal{P}_{i}} \, \Big\{ d(x,c_{i}^{*}) + d(x,g(x)) \Big\} 
\]

\noindent In other words, $x^{*}_{i}$ is a client in $\mathcal{P}_{i}$ that has the minimum total assignment cost to $C$ and $C^{*}$. Let
$g_{i} \coloneqq g(x_{i}^{*}) \in C$ define the representative center of each partition $\mathcal{P}_{i}$. Let $G$ be a multi-set defined as $G \coloneqq \{g_{1},\dotsc,g_{k}\}$. We show that, $G$ is the center set that gives a $\rp{3}{p-1} \cdot (\beta+2)$ approximation for $P$. The proof follows from the following sequence of inequalities:

\begin{align*}
\fair{C'} &= \max_{j \in [\ell]}{\left[ \sum_{i=1}^{k} \costt{g_i, P_j^i}\right]} &&\\
&= \max_{j \in [\ell]}{\left[ \sum_{i=1}^{k} \sum_{x \in P_{j}^{i}} w_{j}(x) \cdot d (g_i,x)^{p}  \right]} &&\\
&\leq \max_{j \in [\ell]}{\left[ \sum_{i=1}^{k} \sum_{x \in P_{j}^{i}} w_{j}(x) \cdot \left( d(x,\cpst{i}) + d(\cpst{i},x_{i}^{*}) + d(x_{i}^{*},g_i) \right)^{p} \right]}, \quad && \textrm{(using triangle inequality)}\\
&\leq \max_{j \in [\ell]}{\left[ \sum_{i=1}^{k} \sum_{x \in P_{j}^{i}} w_{j}(x) \cdot \left(  d(x,\cpst{i}) + d(\cpst{i},x) + d(x,g(x)) \right)^{p} \right]}, \quad && \textrm{(from definition of $g_i$)}\\
&\leq \max_{j \in [\ell]}{\left[ \rp{3}{p-1} \cdot \sum_{i=1}^{k} \sum_{x \in P_{j}^{i}} w_{j}(x) \cdot \left( d(x,\cpst{i}) + d(\cpst{i},x) + d(x,g(x)) \right)  \right]}, \quad && \textrm{(using Fact~\ref{fact:1})}\\
\end{align*}
\vspace{-13mm}
\begin{align*}
\quad \quad\quad\quad\quad \hspace{0.4mm} &\leq \max_{j \in [\ell]}{\left[ \rp{3}{p-1} \cdot  2 \cdot \sum_{i=1}^{k} \sum_{x \in P_{j}^{i}} w_{j}(x) \cdot  d(x,\cpst{i})^{p}  \right]} + \max_{j \in [\ell]}{\left[ \rp{3}{p-1} \cdot \sum_{i=1}^{k} \sum_{x \in P_{j}^{i}} w_{j}(x) \cdot d(x,g(x))^{p}   \right]}&&\\
&=  \max_{j \in [\ell]}{\left[ 2 \cdot \rp{3}{p-1} \cdot \sum_{i=1}^{k} \costt{\cpst{i}, P_j^i}\right]} +  \max_{j \in [\ell]}{\left[ \rp{3}{p-1} \cdot  \costt{C,P_{j}^{i}} \right]}&&\\
&\leq  2 \cdot \rp{3}{p-1} \cdot OPT +  \max_{j \in [\ell]}{\left[ \rp{3}{p-1} \cdot \costt{C,P_{j}^{i}} \right]}&&\\
&\leq 2 \cdot \rp{3}{p-1} \cdot OPT +  \rp{3}{p-1} \cdot \alpha \cdot OPT , &&\hspace{-40mm} \textrm{(using eqn.~\ref{eqn:bound-1})}\\
&= \rp{3}{p-1} \cdot (\alpha+2) \cdot OPT.
\end{align*}
\qed
\end{proof}

\noindent We apply the above lemma for every group $P_j$ individually. That is, we obtain a $\beta$-approximate center set $C_j$ for every group $P_j$. Then, we obtain a multi-set $C_j'$ for each $\mathbb{P}_j$. 

\begin{figure}[h]
\begin{framed}
\ISF~($P,P_1,\dotsc,P_{\ell},w_1,\dotsc,w_{\ell},F,d,k,p,\veps'$) \vspace{2mm}\\
\hspace*{0.3in} {\bf Inputs}: socially fair clustering instance $\mathcal{I} = (P,P_1,\dotsc,P_{\ell},w_1,\dotsc,w_{\ell},F,d,k,p)$ and accuracy $\veps'<1$ \\
\hspace*{0.3in} {\bf Output}: A center set $C \subseteq F$ that is a $(\rp{3}{p-1} \cdot (\rp{3}{p-1} + \beta + 4)+\veps')$-approximate solution to $\mathcal{I}$\vspace*{2mm}\\
\hspace*{0.0mm} (1) \ \ \ For every group $P_j$: \\
\hspace*{0.0mm} (2) \hspace*{0.3in} \ \ \ $C_{j} \gets$ $\beta$-approximate solution of \,$(P_j,F,w_{j},d,k,p)$ \\
\hspace{27mm}\emph{(Algorithm 1 of~\cite{constrained:2020_GJK_FPT} for the weighted point set)}\\
\hspace*{0.0mm} (3) \ \ \ $C \gets \emptyset$ \\
\hspace*{0.0mm} (4) \ \ \ min-cost $ \gets \infty$ \\
\hspace*{0.0mm} (5)\hspace*{0.0in}  \ \ \ For every $k$ sized subset $C_{t}$ of $C_1 \cup \dotsc \cup C_{\ell}$:  \\
\hspace*{0.0mm} (6)\hspace*{0.3in} \ \ \ If $\fair{C_t} < $ min-cost:\\
\hspace*{0.0mm} (7)\hspace*{0.7in} $C \gets C_{t}$\\
\hspace*{0.0mm} (8)\hspace*{0.7in} min-cost $\gets \fair{C_{t}}$\\
\hspace*{0.0mm} (9) \ \  return($C$)
\end{framed}
\vspace*{-4mm}
\caption{An Improved FPT Approximation Algorithm for Socially Fair Clustering Problem}
\label{algorithm:social-fair-improved}
\end{figure}



